SAM2-Adapter: Evaluating & Adapting Segment Anything 2 in Downstream Tasks: Camouflage, Shadow, Medical Image Segmentation, and More

The advent of large models, also known as foundation models, has significantly transformed the AI research landscape, with models like Segment Anything (SAM) achieving notable success in diverse image segmentation scenarios. Despite its advancements, SAM encountered limitations in handling some complex low-level segmentation tasks like camouflaged object and medical imaging. In response, in 2023, we introduced SAM-Adapter, which demonstrated improved performance on these challenging tasks. Now, with the release of Segment Anything 2 (SAM2), a successor with enhanced architecture and a larger training corpus, we reassess these challenges. This paper introduces SAM2-Adapter, the first adapter designed to overcome the persistent limitations observed in SAM2 and achieve new state-of-the-art (SOTA) results in specific downstream tasks including medical image segmentation, camouflaged (concealed) object detection, and shadow detection. SAM2-Adapter builds on the SAM-Adapter's strengths, offering enhanced generalizability and composability for diverse applications. We present extensive experimental results demonstrating SAM2-Adapter's effectiveness. We show the potential and encourage the research community to leverage the SAM2 model with our SAM2-Adapter for achieving superior segmentation outcomes. Code, pre-trained models, and data processing protocols are available at http://tianrun-chen.github.io/SAM-Adaptor/

==> sec/6_More_Results.tex <==
\section{More Results}



==> sec/author.tex <==
\author[1,2]{Tianrun Chen$^{+*}$}
\author[3]{Ankang Lu$^{+}$}
\author[4]{Lanyun Zhu$^{+}$}
\author[1]{Chaotao Ding$^{+}$}
\author[3]{Chunan Yu}
\author[6]{Deyi Ji}
\author[5]{Zejian Li}
\author[2]{Lingyun Sun}
\author[1]{Papa Mao}
\author[3]{Ying Zang$^{*}$}

\affil[1]{KOKONI, Moxin (Huzhou) Tech. Co., LTD, Huzhou, Zhejiang, P.R. China.}
\affil[2]{College of Computer Science and Technology, Zhejiang University, Hangzhou, Zhejiang, P.R. China.}
\affil[3]{School of Information Engineering, Huzhou University, Huzhou, Zhejiang, P.R. China.}
\affil[4]{Information Systems Technology and Design Pillar, Singapore University of Technology and Design, Singapore.}
\affil[5]{School of Software Technology, Zhejiang University, Hangzhou, Zhejiang, P.R. China.}
\affil[6]{School of Information Science and Technology, University of Science and Technology of China, P.R. China.}
\affil[ ]{\{tianrun.chen@zju.edu.cn, 02750@zjhu.edu.cn\}}
\affil[ ]{\textbf{This Work is Built Upon the \href{http://tianrun-chen.github.io/SAM-Adaptor/}{SAM-Adapter - First Available at 14 April, 2023}}}
\affil[ ]{\textbf{TL; DR}. SAM2, enhanced with our new adapter, can replace SAM as the backbone for downstream tasks, establishing new state-of-the-art (SOTA) results!}
\affil[ ]{\small $^+$ Equal Contribution   $^*$ Corresponding Author}
